LLMs in Mobile Apps: Practices, Challenges, and Opportunities

The integration of AI techniques has become increasingly popular in software development, enhancing performance, usability, and the availability of intelligent features. With the rise of large language models (LLMs) and generative AI, developers now have access to a wealth of high-quality open-source models and APIs from closed-source providers, enabling easier experimentation and integration of LLMs into various systems. This has also opened new possibilities in mobile application (app) development, allowing for more personalized and intelligent apps. However, integrating LLM into mobile apps might present unique challenges for developers, particularly regarding mobile device constraints, API management, and code infrastructure. In this project, we constructed a comprehensive dataset of 149 LLM-enabled Android apps and conducted an exploratory analysis to understand how LLMs are deployed and used within mobile apps. This analysis highlights key characteristics of the dataset, prevalent integration strategies, and common challenges developers face. Our findings provide valuable insights for future research and tooling development aimed at enhancing LLM-enabled mobile apps.

==> Backup.tex <==

    
\subsubsection{Feature Additions}
Numerous messages indicate the addition of new features, such as voice input/output, image generation, chat functionalities, and user interface enhancements. These features often aim to improve user experience and expand the app's capabilities.

\textbf{Examples: } \textit{``feat: suppport translate and summary using local ai (\#5858)''} and \textit{``feat: adding GPT-4o''}.

\textbf{Findings: } This is the most common message topic and is an umbrella for many changes. There are a wide range of messages considered to be feature additions, including large overlap with API Integration and Updates surrounding integrating new APIs and updating models. Other popular feature additions include audio transcription and image generation, UI additions such as adding menus to display model options, and back-end changes to the app.

\subsubsection{Refactoring and Code Cleanup}
We find 442 commits involve refactoring code for better organization, readability, and maintainability. This includes renaming variables, restructuring files, and removing unused code, which helps improve the overall code quality.

\textbf{Examples: } \textit{``refactor: Simplify HuggingFace\_API's \_generate method''} and \textit{``refactor: move openai state, store and logic into its own service''}.

\textbf{Findings: } This is the second most common message topic. Many commit messages include the word `refactor', and often involve moving files or code sections, or modifying LLM code.

\subsubsection{Version Updates}
Several messages indicate updates to the app's version, often accompanied by notes on new features, bug fixes, or improvements. This is a common practice in software development to track changes and releases.

\textbf{Examples: } \textit{``Upgrade LangChain.dart to v0.5.0''} and \textit{``Update to v5.2''}.

\textbf{Findings: } Version Updates is the third most common message topic. Most messages that involved some version numbers, seen in the examples, were classified under this topic. 
Many developers used only version numbers or dates as commit messages, which do not provide much information on what updates they are making to the app.

\subsubsection{Bug Fixes}
A significant number of commits are dedicated to fixing bugs, addressing issues like crashes, incorrect API responses, and UI glitches. This is crucial for maintaining app stability and user satisfaction.

\textbf{Examples: } \textit{``fix: local ai enable\/disable (\#6151)''} and \textit{``fix: change chatgpt prompt''}.

\textbf{Findings: } Bug fixes is the fourth most popular commit message topic. Most messages using the words 'bug' or 'fix' are classified under this topic, and usually concern changes to back-end code.

\subsubsection{API Integration and Updates}
Many commits focus on integrating or updating various APIs, particularly those related to OpenAI, DALL-E, and other AI services. This includes adding new endpoints, modifying existing ones, and ensuring compatibility with the latest API specifications.

\textbf{Examples: } \textit{``Integrated OpenAI API as a fallback for unanswered local questions.''} and \textit{``Fixed the model to the latest gpt-3.5-turbo model''}.

\textbf{Findings: } As most of the apps use APIs to access LLMs, many commit messages center around adding new APIs, updating models, or changing infrastructure related to sending or receiving prompts and answers.

\subsubsection{User Interface (UI) Improvements}
Many commits focus on enhancing the user interface, including layout changes, theme updates, and overall design improvements. This is essential for providing a better user experience and making the app more visually appealing.

\textbf{Examples: } ``Make Archive button close realtime session'', ``don't show cost in \$ but in tokens''

\textbf{Findings: } Messages surrounding design are grouped under this topic. Often this involves chat screens, buttons and user options, and API key display.

\subsubsection{Error Handling}
There are numerous mentions of improving error handling mechanisms within the app. This includes adding error messages, handling exceptions, and ensuring that the app can gracefully recover from issues.

\textbf{Examples: } \textit{``update: handle open ai not responding or failing in general with a default message''} and \textit{``Enhanced ai.dart with comments, documentation, and improved error handling''}.

\textbf{Findings: } Error Handling is an infrequent message topic that comes up for messages about error messages, error handling and retries.

\subsubsection{Performance Optimizations}
Some commits focus on optimizing the app's performance, such as improving loading times, reducing memory usage, and enhancing the efficiency of API calls. This is crucial for providing a smooth user experience.

\textbf{Examples: } \textit{``Batch API calls when there is more than 1000 UIDs''} and \textit{``Add more parameters and optimize network module''}.

\textbf{Findings: } This is the third least common topic. Messages that contain the word 'optimize' are grouped into this topic, as well as improvements to prompts such as changes to temperature or token length.

\subsubsection{Localization and Language Support}
Several commits indicate efforts to add or improve localization features, allowing the app to support multiple languages and cater to a broader audience. This includes adding translations and adjusting language settings.

\textbf{Examples: } \textit{``Added support of multiple languages of voice assistant''} and \textit{``detect language from chat response with mlkit and set tts locale to current locale from response text''}.

\textbf{Findings: } This is the second least common topic. As the GPT description states, some apps offer services in multiple languages or translations, which are grouped into this topic.

\subsubsection{Testing and Quality Assurance}
A number of commits mention testing efforts, including unit tests, integration tests, and quality assurance measures. This is important for ensuring that new features and changes do not introduce new bugs or regressions.

\textbf{Examples: } \textit{``chore: have test pass, implement some service test (\#33)''} and \textit{``:white\_check\_mark: model and no stream completions has pass test''}.

\textbf{Findings: } This is the least popular message topic. It is used for any message that mentions testing, and in some cases checking, debugging, or diagnosing, code.
